A Comparison of Statistical and Machine Learning Algorithms for Predicting Rents in the San Francisco Bay Area

Urban transportation and land use models have used theory and statistical modeling methods to develop model systems that are useful in planning applications. Machine learning methods have been considered too 'black box', lacking interpretability, and their use has been limited within the land use and transportation modeling literature. We present a use case in which predictive accuracy is of primary importance, and compare the use of random forest regression to multiple regression using ordinary least squares, to predict rents per square foot in the San Francisco Bay Area using a large volume of rental listings scraped from the Craigslist website. We find that we are able to obtain useful predictions from both models using almost exclusively local accessibility variables, though the predictive accuracy of the random forest model is substantially higher.

==> Tables/describe.tex <==
\begin{tabular}{c | c | c | c | c | c | c | c}
363010.0 & 3.0 & 1.0 & 0.0 & 2.0 & 3.0 & 4.0 & 11.0 \\
363010.0 & 994.0 & 430.0 & 212.0 & 710.0 & 904.0 & 1150.0 & 3600.0 \\
363010.0 & 664.0 & 662.0 & 0.0 & 193.0 & 437.0 & 876.0 & 2317.0 \\
363010.0 & 1455.0 & 712.0 & 0.0 & 1059.0 & 1436.0 & 1803.0 & 3699.0 \\
363010.0 & 133.0 & 148.0 & 0.0 & 27.0 & 81.0 & 166.0 & 528.0 \\
363010.0 & 201.0 & 254.0 & 0.0 & 35.0 & 101.0 & 228.0 & 868.0 \\
363010.0 & 92.0 & 102.0 & 0.0 & 21.0 & 56.0 & 117.0 & 363.0 \\
363010.0 & 226.0 & 189.0 & 0.0 & 79.0 & 186.0 & 327.0 & 755.0 \\
363010.0 & 759.0 & 1295.0 & 0.0 & 43.0 & 220.0 & 748.0 & 5247.0 \\
363010.0 & 6589.0 & 8770.0 & 0.0 & 1206.0 & 3110.0 & 7220.0 & 32501.0 \\
363010.0 & 165285.0 & 117970.0 & 0.0 & 74380.0 & 127551.0 & 236962.0 & 412326.0 \\
363010.0 & 498022.0 & 229898.0 & 37.0 & 322181.0 & 584284.0 & 696465.0 & 787748.0 \\
363010.0 & 333207.0 & 191209.0 & 0.0 & 183445.0 & 300216.0 & 459446.0 & 763247.0 \\
363010.0 & 14010.0 & 18451.0 & 0.0 & 2709.0 & 5754.0 & 20794.0 & 90219.0 \\
363010.0 & 57468.0 & 42489.0 & 0.0 & 27776.0 & 45772.0 & 81072.0 & 201053.0 \\
363010.0 & 106511.0 & 77819.0 & 0.0 & 37199.0 & 93097.0 & 175019.0 & 282688.0 \\
\end{tabular}

==> sections/10-notes.tex <==
Put random notes here





==> sections/tikz-picture-architecture-print-version.tex <==
\tikzstyle{compexpanded}=[inner sep=0pt,minimum size=4mm]
\tikzstyle{comp}=[draw,rectangle,minimum size=4mm]
\tikzstyle{ldots}=[inner sep=0pt,minimum size=4mm]
\tikzstyle{comptitle}=[red, inner sep=0pt,minimum size=4mm]
\tikzstyle{servercomp}=[draw,rectangle,inner sep=0pt,minimum size=4mm]

\begin{tikzpicture}

\node[comptitle] (pdvtitle) at (0, 0.6) {Virtual Personal Data Vaults (PDV)};
\node[comp] (pdv1) at (0, 0) {user$_n$};
\node[comp] (pdv2) at (5.2, 0) {user$_{n+1}$};
\node[ldots] (pdv3) at (7.3, 0) {$\ldots$};
\node[comp] (pdv4) at (-5, 0) {user$_{n-1}$};
\node[ldots] (pdv5) at (-7, 0) {$\ldots$};

% BEGIN: CREATE corner points
\path (pdv5.west |- pdvtitle.north)+(-0.1,0.2) node (allpdnw) {};
\path (pdv1.south -| pdv3.east)+(+0.1,-0.2) node (allpdse) {};
% END: CREATE corner points

\node[comptitle] (intaketitle) at (-5.5, -1.3) {intake pipeline};

% BEGIN: CREATE corner points
\path (intaketitle.west |- intaketitle.north)+(-0.1,0.05) node (intakenw) {};
\path (intaketitle.south -| intaketitle.east)+(0.1,-0.1) node (intakese) {};
% END: CREATE corner points

\node[comptitle] (iotitle) [right of=intaketitle, anchor=west, node distance=4em] {I/O};
\node[comptitle] (api) [right of=iotitle, anchor=west, node distance=4em] {api + auth};

% BEGIN: CREATE corner points
\path (iotitle.west |- iotitle.north)+(-0.1,0.05) node (ionw) {};
\path (iotitle.south -| iotitle.east)+(0.1,-0.1) node (iose) {};
% END: CREATE corner points

\node[comptitle] (resulttitle) [right of=api, anchor=west, node distance=4em] {result};
\node[comptitle] (aggtitle) [above of=resulttitle, anchor=south, node distance=.6em] {aggregate};

% BEGIN: CREATE corner points
\path (resulttitle.west |- resulttitle.north)+(-0.1,0.05) node (resultnw) {};
\path (resulttitle.south -| resulttitle.east)+(0.1,-0.1) node (resultse) {};
% END: CREATE corner points

\node[comptitle] (exttitle) [right of=resulttitle, anchor=west, node distance=4em] {external};

% BEGIN: CREATE corner points
    \path (exttitle.west |- exttitle.north)+(-0.1,0.05) node (extnw) {};
    \path (exttitle.south -| exttitle.east)+(0.1,-0.1) node (extse) {};
% END: CREATE corner points

% BEGIN: CREATE corner points
    \path (resultnw.west |- resultnw.north)+(-0.05,+0.35) node (aggnw) {};
    \path (exttitle.center |- resultse.south)+(+0.05,-0.05) node (aggse) {};
% END: CREATE corner points

\node[comptitle] (servertitle) at (0,1.3) {Server};

% \path (allpdnw.west |- aggse.south)+(+0.1,-0.05) node (apinw) {};
% \path (allpdse.east |- apinw.north)+(-0.1,-0.7) node (apise) {};

% \path [fill=green!10,line width=4mm,join=round]
%     (apinw) rectangle node (api) {api + auth} (apise);
\path (api.west |- api.north)+(-0.1,0.05) node (apinw) {};
\path (api.south -| api.east)+(0.1,-0.1) node (apise) {};

% BEGIN: CREATE corner points
\path (allpdnw.west |- servertitle.north)+(-0.1,+0.2) node (servernw) {};
\path (allpdse.east |- apise.south)+(+0.1,-0.2) node (serverse) {};
% END: CREATE corner points

% Now actually draw the background
\begin{pgfonlayer}{background}
    % server
    \path [fill=yellow!50,line width=4mm,join=round]
            (servernw) rectangle (serverse);

    % Personal data store
    \path [fill=blue!10,line width=4mm,join=round]
            (allpdnw) rectangle (allpdse);

    % Aggreate rectangle
    \path [fill=magenta!10,line width=4mm,join=round]
        (aggnw) rectangle (aggse);

    % intake
    \path [fill=green!10,line width=4mm,join=round]
        (intakenw) rectangle (intakese);

    % I/O
    \path [fill=green!10,line width=4mm,join=round]
        (ionw) rectangle (iose);

    % result
    \path [fill=green!10,line width=4mm,join=round]
        (resultnw) rectangle (resultse);
    % ext
    \path [fill=green!10,line width=4mm,join=round]
        (extnw) rectangle (extse);

    % api
    \path [fill=green!10,line width=4mm,join=round]
        (apinw) rectangle (apise);
\end{pgfonlayer}

% now for the phone
\node[comp] (transnotify) at (-6.50, -3.5) {prompt};
\node[comp] (cache) [right of=transnotify, anchor=west, node distance=40pt] {buffer};
\node[comp] (sense) [right of=cache, anchor=west, node distance=40pt] {sense};
\node[comp] (sync) [right of=sense, anchor=west, node distance=50pt] {sync};
\node[comp] (auth) [right of=sync, anchor=west, node distance=60pt] {auth};
\node[comptitle] (nativetitle) [above of=sense, anchor=south, node distance=10pt] {Native plugins};

% BEGIN: CREATE corner points
\path (transnotify.west |- nativetitle.north)+(-0.1,0.05) node (nativenw) {};
\path (auth.south -| auth.east)+(0.1,-0.1) node (nativese) {};
% END: CREATE corner points

% now for the phone
\node[comp] (diary) at (-6.50, -5) {diary};
\node[comp] (game) [right of=diary, anchor=west, node distance=40pt] {game};
\node[comp] (dashboard) [right of=game, anchor=west, node distance=40pt] {dashboard};
\node[comp] (heatmap) [right of=dashboard, anchor=west, node distance=40pt] {heatmap};
\node[comp] (controls) [right of=heatmap, anchor=west, node distance=40pt] {control};
\node[comptitle] (displaytitle) [above of=dashboard, anchor=south, node distance=10pt] {Display layer (HTML + javascript)};

% BEGIN: CREATE corner points
\path (diary.west |- displaytitle.north)+(-0.1,0.05) node (displaynw) {};
\path (controls.south -| controls.east)+(0.1,-0.1) node (displayse) {};
% END: CREATE corner points

\node[comptitle] (phonetitle) [above of=nativetitle, anchor=south, node distance=10pt] {Phone};

% BEGIN: CREATE corner points
\path (nativenw.west |- phonetitle.north)+(-0.1,0.05) node (phonenw) {};
\path (displayse.south -| displayse.east)+(0.1,-0.1) node (phonese) {};
% END: CREATE corner points

\begin{pgfonlayer}{background}
    % phone
    \path [fill=yellow!50,line width=4mm,join=round]
            (phonenw) rectangle (phonese);

    % native
    \path [fill=orange!10,line width=4mm,join=round]
        (nativenw) rectangle (nativese);

    % display 
    \path [fill=orange!10,line width=4mm,join=round]
        (displaynw) rectangle (displayse);
\end{pgfonlayer}

\path (phonese.east |- phonenw.north)+(+0.1,-0.1) node (browsernw) {};
\path (phonese.south -| serverse.east)+(-0.1,+0.1) node (browserse) {};

\path [fill=yellow!50,line width=4mm,join=round]
    (browsernw) rectangle (browserse);

\path (browsernw.west |- browsernw.north)+(0.8,0.5) node (browsertitleloc) {};
\node[comptitle] (browsertitle) [below of=browsertitleloc] {Browser};
\node[compexpanded] (browserhtml) [below of=browsertitle] {HTML};
\node[compexpanded] (browserjs) [below of=browserhtml] {+ js};

\path (phonenw.west |- phonese.south)+(+0.1,-0.1) node (personnw) {};
\path (browserse.east |- personnw.north)+(-0.1,-0.7) node (personse) {};

\path [fill=red!50,line width=4mm,join=round]
    (personnw) rectangle node (person) {Person} (personse);

\end{tikzpicture}


==> sections/tikz-picture-structure.tex <==
\tikzstyle{collection}=[font=\tiny,draw,rectangle,text width=3.25cm, minimum width=3.25cm,minimum height=1cm]
\tikzstyle{integration}=[font=\tiny,draw,rectangle,text width=1cm, minimum width=1cm,minimum height=1.5cm]
\tikzstyle{processing}=[font=\tiny,draw,rectangle,text width=3cm, minimum width=3cm,minimum height=1cm]
\tikzstyle{aggregation}=[font=\tiny,text centered,draw,rectangle,text width=8.5cm, minimum width=8.5cm,minimum height=1cm]
\tikzstyle{external}=[font=\tiny,text width=2cm, minimum width=2cm]

\begin{tikzpicture}[>=stealth]

% draw the central "storage" element
% center text
\node[font=\tiny] (storage) at (0,0) {STORAGE};
% lines on the sides
\draw (-1.25,0.25) -- (-1.25, -0.25);
\draw (1.25,0.25) -- (1.25,-0.25);
% arcs
\draw (-1.25,-.25) arc (180:360:1.25cm and .11cm);
\draw (-1.25,.25) arc (180:360:1.25cm and .11cm);
\draw (-1.25,.25) arc (180:0:1.25cm and .11cm);
% end central "storage" element

% draw all the nodes in the mobilityscope
\node[collection] (background) at (-1.75, 1.5) {traveler-specific background sensing};
\node[collection] (semantic) at (2, 1.5) {traveler-entered semantic/ perceptual data};
\node[processing] (processing) at (0,-1.25) {services/ processing/ inference};
\node[integration] (input) at (-2.5, -0.25) {input sources};
\node[integration] (output) at (2.5, -0.25) {output APIs};

% Add input and output arrows
\draw[->] (-4.5,1.5) to [bend left] node[external] {transit schedules} (input.west);
\draw[->] (-4.5,0) to node[external, below] {freeway sensors} (input.west);
\draw[->] (-4.5,-1.5) to [bend right] node[external, below] {\textbf{\vdots}} (input.west);

\draw[<-] (4.5,1.5) to [bend left] node[right,external] {points} (output.east);
\draw[<-] (4.5,0) to node[right,external] {trips} (output.east);
\draw[<-] (4.5,-1.5) to [bend right] node[right,external] {\textbf{\vdots}} (output.east);

% Add edges
\path[<->] (background) edge (storage)
           (semantic) edge (storage);
\path[->] (input) edge (storage)
          (storage) edge (output)
          (processing) edge[bend left] (storage)
          (storage.south) edge[bend left] (processing)
          (input.south) edge[bend right] (processing.west)
          (processing.east) edge[bend right] (output.south);

% Draw the background
\begin{pgfonlayer}{background}
    % last layer, don't care if it is filled
    \draw (-3.5,2) rectangle (4.5, -2.5);
    % middle layer, filled and drawn
    \filldraw[fill=white,draw=black] (-3.75,2.25) rectangle (4.25, -2.25);
    % top layer, filled and drawn
    \filldraw[fill=white,draw=black] (-4.0,2.5) rectangle (4.0, -2);
\end{pgfonlayer}

% Draw the aggregation layer
\node[aggregation](aggregation) at (0.25, -3.5) {aggregation};
\draw[->] (-3,-2) -- (aggregation);
\draw[->] (-2,-2.25) -- (aggregation);
\draw[->] (-1, -2.5) -- (aggregation);
\node[external] at (1, -2.75) {\textbf{\ldots}};

% Draw the people

% Traveler at the top: (0, 3.25)
\draw (0, 3.25) circle (0.1)
       +(0, -0.1) -- +(0, -0.5)
       +(0, -0.2) -- +(-0.2, -0.3)
       +(0, -0.2) -- +(0.2, -0.3)
       +(0, -0.4) -- +(-0.2, -0.5)
       +(0, -0.4) -- +(0.2, -0.5);
\node[font=\tiny] (traveler) at (1, 3) {Traveler};

% Planner at the bottom: 0, -4.5
\draw (0, -4.5) circle (0.1)
       +(0, -0.1) -- +(0, -0.5)
       +(0, -0.2) -- +(-0.2, -0.3)
       +(0, -0.2) -- +(0.2, -0.3)
       +(0, -0.4) -- +(-0.2, -0.5)
       +(0, -0.4) -- +(0.2, -0.5);
\node[font=\tiny] (planner) at (1, -4.75) {Planner};

% Small travelers at the side
\draw (4.05, 2.80) circle (0.05)
       +(0, -0.05) -- +(0, -0.25)
       +(0, -0.1) -- +(-0.1, -0.15)
       +(0, -0.1) -- +(0.1, -0.15)
       +(0, -0.2) -- +(-0.1, -0.25)
       +(0, -0.2) -- +(0.1, -0.25);

\draw (4.30, 2.55) circle (0.05)
       +(0, -0.05) -- +(0, -0.25)
       +(0, -0.1) -- +(-0.1, -0.15)
       +(0, -0.1) -- +(0.1, -0.15)
       +(0, -0.2) -- +(-0.1, -0.25)
       +(0, -0.2) -- +(0.1, -0.25);

\node at (3.70, 2.65) {\textbf{\ldots}};

% Edges to/from people
\path[->] (traveler) edge (background) edge (semantic)
      (output.east) edge[bend right=90,looseness=1.5] (traveler.east)
      (-3,-4) edge[bend right] node[above,font=\tiny] {counts} (-.25, -4.7)
      (-1.5,-4) edge[bend right] node[above,font=\tiny] {speeds} (-.25, -4.5)
      (-0.25,-4) edge node {\textbf{\ldots}} (planner)
      (0.25,-4) edge node {\textbf{\ldots}} (planner)
      (3,-4) edge[bend left] node[above,font=\tiny] {models} (planner);

\end{tikzpicture}


==> tabletest.tex <==
'\\begin{tabular}{lrrrrrrrr}\n\\toprule\n{} &     count &      mean &       std &    min &       25\\% &       50\\% &       75\\% &       max \\\\\n\\midrule\nrent\\_sqft           &  363010.0 &       3.0 &       1.0 &    0.0 &       2.0 &       3.0 &       4.0 &      11.0 \\\\\nres\\_sqft\\_per\\_unit   &  363010.0 &     994.0 &     430.0 &  212.0 &     710.0 &     904.0 &    1150.0 &    3600.0 \\\\\nunits\\_500\\_walk      &  363010.0 &     664.0 &     662.0 &    0.0 &     193.0 &     437.0 &     876.0 &    2317.0 \\\\\nsqft\\_unit\\_500\\_walk  &  363010.0 &    1455.0 &     712.0 &    0.0 &    1059.0 &    1436.0 &    1803.0 &    3699.0 \\\\\nrich\\_500\\_walk       &  363010.0 &     133.0 &     148.0 &    0.0 &      27.0 &      81.0 &     166.0 &     528.0 \\\\\nsingles\\_500\\_walk    &  363010.0 &     201.0 &     254.0 &    0.0 &      35.0 &     101.0 &     228.0 &     868.0 \\\\\nelderly\\_hh\\_500\\_walk &  363010.0 &      92.0 &     102.0 &    0.0 &      21.0 &      56.0 &     117.0 &     363.0 \\\\\nchildren\\_500\\_walk   &  363010.0 &     226.0 &     189.0 &    0.0 &      79.0 &     186.0 &     327.0 &     755.0 \\\\\njobs\\_500\\_walk       &  363010.0 &     759.0 &    1295.0 &    0.0 &      43.0 &     220.0 &     748.0 &    5247.0 \\\\\njobs\\_1500\\_walk      &  363010.0 &    6589.0 &    8770.0 &    0.0 &    1206.0 &    3110.0 &    7220.0 &   32501.0 \\\\\njobs\\_10000          &  363010.0 &  165285.0 &  117970.0 &    0.0 &   74380.0 &  127551.0 &  236962.0 &  412326.0 \\\\\njobs\\_25000          &  363010.0 &  498022.0 &  229898.0 &   37.0 &  322181.0 &  584284.0 &  696465.0 &  787748.0 \\\\\npop\\_10000           &  363010.0 &  333207.0 &  191209.0 &    0.0 &  183445.0 &  300216.0 &  459446.0 &  763247.0 \\\\\npop\\_black\\_10000     &  363010.0 &   14010.0 &   18451.0 &    0.0 &    2709.0 &    5754.0 &   20794.0 &   90219.0 \\\\\npop\\_hisp\\_10000      &  363010.0 &   57468.0 &   42489.0 &    0.0 &   27776.0 &   45772.0 &   81072.0 &  201053.0 \\\\\npop\\_asian\\_10000     &  363010.0 &  106511.0 &   77819.0 &    0.0 &   37199.0 &   93097.0 &  175019.0 &  282688.0 \\\\\n\\bottomrule\n\\end{tabular}\n'
